Watermarking PRFs against Quantum Adversaries

We initiate the study of software watermarking against quantum adversaries. A quantum adversary generates a quantum state as a pirate software that potentially removes an embedded message from a classical marked software. Extracting an embedded message from quantum pirate software is difficult since measurement could irreversibly alter the quantum state. In this work, we define secure watermarking PRFs for quantum adversaries (unremovability against quantum adversaries). We also present two watermarking PRFs as follows. - We construct a privately extractable watermarking PRF against quantum adversaries from the quantum hardness of the learning with errors (LWE) problem. The marking and extraction algorithms use a public parameter and a private extraction key, respectively. The watermarking PRF is unremovable even if adversaries have (the public parameter and) access to the extraction oracle, which returns a result of extraction for a queried quantum circuit. - We construct a publicly extractable watermarking PRF against quantum adversaries from indistinguishability obfuscation (IO) and the quantum hardness of the LWE problem. The marking and extraction algorithms use a public parameter and a public extraction key, respectively. The watermarking PRF is unremovable even if adversaries have the extraction key (and the public parameter). We develop a quantum extraction technique to extract information (a classical string) from a quantum state without destroying the state too much. We also introduce the notion of extraction-less watermarking PRFs as a crucial building block to achieve the results above by combining the tool with our quantum extraction technique.

==> section/simple_watermarking.tex <==
% !TEX root = ../main.tex


\newcommand{\Drev}{D^{\mathtt{rev}}}
\newcommand{\cPrev}{\cP^{\mathtt{rev}}}
\newcommand{\ELWMPRF}{\mathsf{ELWMPRF}}

\section{Watermarkable PRF from Extraction-Less Watermarkable PRF}\label{sec:simple_watermarkable_prf}




%
%\subsection{Mark-Embedding Scheme}\label{sec:simple_mark_embedding}
%Watermarking scheme for PPPRF. In this scheme, a circuit can be seen as a master secret key of PRF.
%\begin{description}
% \item[$\Gen(1^\secp)$:] $ $
%
% \begin{itemize}
% \item Choose $(x_i,y_i) \chosen \zo{n}\times\zo{m} $ for $i = 1,\ldots,\ell$.
% \item Output $\mk = \ek \seteq (\setbk{x_i}_i,\setbk{y_i}_i)$.
% \end{itemize}
%\item[$\Mark (\mk,\msk)$:] $ $
%\begin{itemize}
%	\item Parse $\mk =(\setbk{x_i}_i,\setbk{y_i}_i)$.
%\item Generate $\sk \lrun \ppprf.\program(\msk,\setbk{x_i}_i,\setbk{y_i}_i)$.
%\item Output $\tlC \seteq \sk$.
%\end{itemize}
%\item[$\qExtract (\ek,\qstate{C}^{\prime})$:]$ $
%\begin{itemize}
%\item Compute $\tlp \lrun \API_{\cP,D_{\ek}}^{\epsilon,\delta}(\qstate{C}^\prime)$.
%\item Output $\marked$ if $\tlp \ge 1/\ell$ and otherwise $\unmarked$.
%\end{itemize}
%\item[Distribution $D_{\ek}$:]$ $
%\begin{itemize}
%    \item Parse $\ek = \setbk{x_i,y_i}_{i}$.
%    \item Generate $\sk \lrun \ppprf.\program(\msk,\setbk{x_i}_i,\setbk{y_i}_i)$.
%\item Choose $i \chosen [\ell]$.
%\item Output $(x_i,\ppprf.\peval(\sk,x_i),\sk)$.
%\end{itemize}
%For an evaluator in its initial state and for a given $(x,y)$, the corresponding measurement $\cP_{(x,y)}$ outputs $1$ when the evaluator would output $y$.
%\end{description}
%
%We define another distribution $\hat{D}_{\ek}$ as follows.
%\begin{description}
%\item[Distribution $\hat{D}_{\ek}$:]$ $
%\begin{itemize}
%    \item Parse $\ek = \setbk{x_i,y_i}_i$.
%    \item Choose $x^\prime_i \chosen \zo{n}$ for $i\in[\ell]$.
%    \item Generate $\sk \lrun \ppprf.\program(\msk,\setbk{x^\prime_i}_i,\setbk{y_i}_i)$
%\item Choose $i\chosen [\ell]$.
%\item Output $(x_i, \ppprf.\peval(\msk,x_i),\sk)$.
%\end{itemize}
%\end{description}
%
%
%
%
%
%For any QPT adversary $\qA$, we define the following experiment, $\expt{\qA}{real}(\secp)$.
% % and $\expt{\qA}{rand}(\secp)$.  
%\paragraph{$\expt{\qA}{real}(\secp)$:}
%\begin{enumerate} 
%\setlength{\parskip}{0.5mm}
%\setlength{\itemsep}{0.5mm}
%    \item Generate $\ek=\mk=(\setbk{x_i}_i,\setbk{y_i}_i) \lrun \Gen (1^\secp)$
%    \item Compute $\msk \lrun \ppprf.\Setup(1^\secp)$ and $\tlC \lrun \ppprf.\program(\msk,\setbk{x_i}_i,\setbk{y_i}_i)$.
%    \item Run $\qstate{C}^\ast_{\mathsf{real}} \lrun \qA(\tlC)$
%    \item Set $\hatp_{}^{\sfgood} \seteq \API_{\cP,D_{\ek}}^{\epsilon,\delta}(\qstate{C}_{\mathsf{real}}^\ast)$ and $\hatp_{}^{\sflive} \seteq \API_{\cP,\hat{D}_{\ek}}^{\epsilon,\delta}(\qstate{C}_{\mathsf{real}}^\ast)$.
%    \end{enumerate}
%
%% \paragraph{$\expt{\qA}{rand}(\secp,\coin)$:}
%% \begin{enumerate} 
%% \setlength{\parskip}{0.5mm}
%% \setlength{\itemsep}{0.5mm}
%%     \item $\ek=\mk=(\setbk{x_i}_i,\setbk{y_i}_i) \lrun \Gen (1^\secp)$
%%     \item Choose $x_i^\prime$ for $i\in[\ell]$.
%%     \item $\msk \lrun \ppprf.\Setup(1^\secp)$ and $\tlC^\prime \lrun \ppprf.\program(\msk,\setbk{x_i^\prime}_i,\setbk{y_i}_i)$.
%%     \item $\qstate{C}_{\mathsf{rand}}^\ast \lrun \qA(\tlC^\prime)$.
%%     \item Finally, we set $\hatp_{\mathsf{rand}}^{\sfgood}\seteq \API_{\cP,D_{\ek}}^{\epsilon,\delta}(\qstate{C}_\mathsf{rand}^\ast)$ if $\coin=1$, otherwise $\hatp_{\mathsf{rand}}^{\sflive} \seteq \API_{\cP,D_{\msk}}^{\epsilon,\delta}(\qstate{C}_{\mathsf{rand}}^\ast)$.
%% \end{enumerate}
%
%
%\begin{lemma}\label{lem:sim_ek_ppprf_privacy}
%Assume that programmable PRF $\PRF$ satisfies privacy. Then, for all QPT $\qA$, it holds that
%\[
%D_{\ek} \cind \hat{D}_{\ek}.
%\]
%\end{lemma}
%\begin{proof}
%If these distributions are distinguishable, we can construct a distinguisher $\cD$ for the privacy of $\PRF$.
%\end{proof}
%
%
%By using~\cref{cor:cind_sample_api} (\cite[Corollary 6.9]{TCC:Zhandry20}) with~\cref{lem:sim_ek_ppprf_privacy}, we obtain the lemma below.
%\begin{lemma}\label{lem:cind_dist_API}
%If $\PRF$ is a programmalbe PRF that satisifes privacy, $\shiftdis{3\epsilon}(\API_{\cP,D_{\ek}}^{\epsilon,\delta}, \API_{\cP,\hat{D}_{\ek}}^{\epsilon,\delta}) \le 2\delta + \negl(\secp)$.
%\end{lemma}
%\begin{proof}
%We can immeditely obtain the lemma by using~\cref{cor:cind_sample_api,lem:sim_ek_ppprf_privacy}.
%\end{proof}
%By the definition of $D_{\ek}$ and $\hat{D}_{\ek}$, it holds $\Pr[\Live\text{ happens}] = p_{}^{\sflive}$ and $\shiftdis{\epsilon}(\hatp_{}^{\sflive},p_{}^{\sflive}) \le \delta $.
%
%By the admissibility, $p_{}^{\sflive}\ge \epsilon^\ast$. We set $\epsilon^\ast - 1/\ell \ge \epsilon^\ast (1- 1/\secp) \ge 4\epsilon$.
%
%Now, we assume that
%\[
%\hatp_{\mathsf{real}}^{\sfgood} < 1/\ell. % \API_{\cP,\hat{D}_{\ek}}^{\epsilon,\delta}(\qstate{C}^\ast) \ge \epsilon, ~~~
%\]
%happens with non-negligible probability $\nu$.
%That is, $\qA$ breaks the unremovability with probability $\nu$.
%By the triangle-like inequality, the definition and parameter setting, we have
%\[
%\shiftdis{\epsilon^\ast -1/\ell}(p^{\sflive},\hatp^{\sfgood}) \le \shiftdis{4\epsilon}(p^{\sflive},\hatp^{\sfgood}) \le \shiftdis{\epsilon}(p^{\sflive},\hatp^{\sflive}) + \shiftdis{3\epsilon}(\hatp^{\sflive},\hatp^{\sfgood}).
%\]
%We obtain
%\[
%\shiftdis{3\epsilon}(\hatp_{}^{\sflive}, \hatp_{}^{\sfgood}) \ge \nu - \delta.\label{eq:good_live_diff}
%\]
%
%
%On the other hand, by~\cref{lem:cind_dist_API}, we obtain
%\[
%\shiftdis{3\epsilon}(\hatp_{}^{\sflive}, \hatp_{}^{\sfgood}) \le \negl(\secp)+ 2\delta.\label{eq:diff_live_good_diff_API}
%\]
%\cref{eq:diff_live_good_diff_API} contradict to~\cref{eq:good_live_diff} since $\epsilon^\ast \ge \frac{1}{\poly(\secp)}$, $\nu$ is non-negligible, and we can set $\delta = \negl(\secp)$.
%
%Thus, our assumption $\hatp_{}^{\sfgood}=0$ happens with non-negligible probability is false and the unremobavility holds.

\subsection{Construction}\label{sec:wmprf-from-elwmprf-const}
Let $\ELWMPRF=(\Setup,\Gen,\Eval,\Mark,\KeyExtract, \Sim)$ be an extraction-less watermarkable PRF scheme whose message space is $\bit^{\mklen+1}$.
We construct a watermarkable PRF scheme $\WMPRF=(\WM.\Setup,\WM.\Gen,\WM.\Eval,\WM.\Mark,\qExtract)$ whose message space is $\bit^{\mklen}$ as follows. We use $\Setup$, $\Gen$, and $\Eval$ as $\WM.\Setup$, $\WM.\Gen$, and $\WM.\Eval$, respectively.
Also, we construct $\WM.\Mark$ and $\qExtract$ as follows.

%We need to set the threshold $\gamma$ so that $\gamma - \abs{\msg} \cdot \epsilon \ge 1/\ell$ and $1/\ell \le \gamma < 2/\ell$.
%This condition is equal to $\epsilon < \frac{1}{\ell\cdot \abs{\msg}}$. Here, $\ell = \Omega(\frac{\secp}{\epsilon^\ast})$, $\epsilon$ is an inverse of a polynomial, and $\epsilon^\ast \ge \frac{1}{\poly(\secp)}$.
\begin{description}

% \item[$\Gen(1^\secp)$:] $ $
%
% \begin{itemize}
% \item Choose $(\mv{x}_{i,b},\mv{y}_{i,b}) \chosen (\zo{n})^\ell \times(\zo{m})^\ell $ for $i = 1,\ldots,\abs{\msg}$ and $b\in\zo{}$.
% \item Output $\mk = \ek \seteq \setbk{\ek_{i,b}}_{i,b} $ where $\ek_{i,b} \seteq (\mv{x}_{i,b},\mv{y}_{i,b})$.
% \end{itemize}
\item[$\WM.\Mark (\pp,\prfk, \msg)$:] $ $
\begin{itemize}
\item Output $\tlC \gets \Mark(\pp,\prfk,\msg\|0)$.
\end{itemize}
\item[$\qExtract^{\Oracle{wprf}}(\ek,\qstate{C}^{\prime})$:]$ $
\begin{itemize}
\item Let $\epsilon'=\epsilon/4(\ell+1)$ and $\delta'=2^{-\lambda}$.
\item Parse $(U,\rho)\gets\qstate{C}'$.
\item Compute $\prfk\gets\KeyExtract^{\Oracle{wprf}}(\ek)$.
\item Compute $\tlp_{\ell+1} \gets \API_{\cP,D_{\ell+1}}^{\epsilon' ,\delta'}(\rho)$. If $\tlp_{\ell+1}<\frac{1}{2}+\epsilon-4\epsilon'$, return $\unmarked$. Otherwise, letting $\rho_0$ be the post-measurement state, go to the next step.
\item For all $i \in [\ell]$, do the following
\begin{enumerate}
\item Compute $\tlp_{i} \gets \API_{\cP,D_{i}}^{\epsilon' ,\delta'}(\rho_{i-1})$. Let $\rho_i$ be the post-measurement state.
\item If $\tlp_i>\frac{1}{2}+\epsilon-4(i+1)\epsilon'$, set $\msg'_i=0$. If $\tlp_i<\frac{1}{2}-\epsilon+4(i+1)\epsilon'$, set $\msg'_i=1$. Otherwise, exit the loop and output $\msg'=0^{\ell+1}$.
%\item Compute $\tlt_{i,0} \lrun \ATI_{\cP,D_{\ek_{i,0}},\gamma - (i-1)\epsilon}^{\epsilon ,\delta}(\qstate{C}^\prime)$.
%\item If $\tlt_{i,0}=1$, redefine $\qstate{C}^\prime \seteq \recover(\qstate{C}^\prime)$. Otherwise, leave $\qstate{C}^\prime$ as it is.\ryo{$\tlt_{i,b} =1$ means approximate probability is less than $1/\ell$, which is the threshold.}
%\item Compute $\tlt_{i,1} \lrun \ATI_{\cP,D_{\ek_{i,1}},\gamma - (i-1)\epsilon}^{\epsilon,\delta}(\qstate{C}^\prime)$.
%\item If $\tlt_{i,1}=1$, redefine $\qstate{C}^\prime \seteq \recover(\qstate{C}^\prime)$. Otherwise, leave $\qstate{C}^\prime$ as it is.
%\item Set $\msg_i \seteq b$ if $\tlt_{i,b} = 0 \land \tlt_{i,1-b}=1$. Otherwise, $\msg_i \seteq \bot$.
\end{enumerate}
\item Output $\msg'=\msg'_1 \concat \cdots \concat \msg'_{\ell}$.
\end{itemize}
\end{description}

The distribution $D_i$ is defined as follows for every $i\in[\ell]$.
\begin{description}
\item[Distribution $D_{i}$:]$ $
\begin{itemize}
    \item Generate $(\gamma,x,y)\gets\Sim(\prfk,i)$.
    \item Output $(\gamma,x,y)$.
\end{itemize}
\end{description}
%For an evaluator in its initial state and for a given $(x,y)$, the corresponding measurement $\cP_{(x,y)}$ outputs $1$ when the evaluator would output $y$.
%More precisely, define $(P_{f,x},Q_{f,x})$ be a projective measurement that computes the quantum program $f$ (here, $f=\qstate{C}^\prime$ or expected to be $\ppprf.\Eval(\msk,\cdot)$) on inpute $x$, and checks in superposition that if the quantum circuit outputs correct $f(x)$. Let $V_{f,x}$ be a projection that checks if in superposition, the first register is equal to $f(x)$. We have $P_{f,x}=V_{f,x}U_{f,x}$ and $Q_{f,x}=\mat{I}-P_{f,x}$.


We define another distribution $\Drev_i$ as follows for every $i\in[\ell]$, which are used in the security proof.
\begin{description}
\item[Distribution $\Drev_{i}$:]$ $
\begin{itemize}
    \item Generate $(\gamma,x,y)\gets\Sim(\prfk,i)$.
    \item Output $(1\oplus\gamma,x,y)$.
\end{itemize}
\end{description}

\fuyuki{We see that $(P_{\Drev_i(r)},Q_{\Drev_i(r)})=(Q_{D_i(r)},P_{D_i(r)})$. We use this fact in the proof.}

\subsection{Security Proof}


%For any QPT adversary $\qA$, we define the following experiment, $\expt{\qA}{real}(\secp)$.
%\paragraph{$\expt{\qA}{real}(\secp)$:}
%\begin{enumerate} 
%\setlength{\parskip}{0.5mm}
%\setlength{\itemsep}{0.5mm}
%    \item Generate $\mk=\ek=(\setbk{\mv{x}_{i,b}}_{i,b},\setbk{\mv{y}_{i,b}}_{i,b}) \lrun \Gen (1^\secp)$
%    \item Compute $\msk \lrun \ppprf.\Setup(1^\secp)$.
%    \item Receive $\msg^\ast \lrun \qA(1^\secp)$ and compute $\tlC \lrun \ppprf.\program(\msk,\setbk{\mv{x}_{i,\msg^\ast[i]}}_{i\in [\abs{\msg}]},\setbk{\mv{y}_{i,\msg^\ast[i]}}_{i\in[\abs{\msg}]})$.
%    \item Run $\qstate{C}^\ast_{\mathsf{real}} \lrun \qA(\tlC)$.
%    \item Set $\hatb_{i,b}^{\sfgood} \seteq \ATI_{\cP,D_{\ek_{i,b}},\gamma-\epsilon}^{\epsilon,\delta}(\qstate{C}_{\mathsf{real}}^\ast)$ and $\hatb_{i,b}^{\sflive} \seteq \ATI_{\cP,\hat{D}_{\ek_{i,b}},\gamma-\epsilon}^{\epsilon,\delta}(\qstate{C}_{\mathsf{real}}^\ast)$.
%    \end{enumerate}
%
%Since $\mv{x}_{i,b}$ and $\mv{y}_{i,b}$ are completely independent of $\mv{x}_{i,1-b}$ and $\mv{y}_{i,1-b}$, respectively, $\qA$ has no information about $\mv{x}_{i,1-\msg^\ast[i]}$ and $\mv{y}_{i,1-\msg^\ast[i]}$. More precisely, $\qstate{C}^\ast$ is independent of $\mv{x}_{i,1-\msg^\ast[i]}$ and $\mv{y}_{i,1-\msg^\ast[i]}$ since we can defer choosing $\mv{x}_{i,1-\msg^\ast[i]}$ and $\mv{y}_{i,1-\msg^\ast[i]}$ after we receive $\qstate{C}^\ast$. Thus, $b_{i,1-\msg^\ast[i]}^{\sfgood} =1$ with probability greater than $1 - \frac{\ell}{2^m}$ by union bound.






Let $\qA$ be a QPT adversary attacking the $\epsilon$-unremovability of $\WMPRF$.
%We prove this theorem using hybrid games.
The description of  $\expt{\qA}{nrmv}(\secp,\epsilon)$ is as follows.

\begin{enumerate}
\item The challenger generates $(\pp,\ek) \chosen \Setup(1^\secp)$ and gives $\pp$ to the adversary $\qA$.
$\qA$ send $\msg\in\bit^\mklen$ to the challenger.
The challenger generates $\prfk\gets\Gen(\pp)$, computes $\tlC\gets\Mark(\pp,\prfk,\msg\|0)$, and sends $\tlC$ to $\qA$.

\item $\qA$ can access to the following oracle.
\begin{description}
%\item[$\Oracle{eval}$:]On input $x$, it returns $\Eval(\prfk,x)$.\fuyuki{To Do:remove.}
\item[$\Oracle{ext}$:]On input $(x_i,y_i)_{i\in[\qext]}$ and a quantum program $\qstate{C}$, it returns $\qExtract^{\Oracle{wprf}}(\ek,\qstate{C})$, where $\Oracle{wprf}$ is simulated by using $(x_i,y_i)_{i\in[\qext]}$.
\end{description}


\item Finally, the adversary outputs a quantum program $\qstate{C}'=(\rho,U)$.
\end{enumerate}

We define $D$, $\cP$, $\cM_D$, and the three events $\Live$, $\GoodExt$, and $\BadExt$ in the same way as \cref{def:watermarking_prf}.

%Let $D$ be the following distribution.
%\begin{description}
%\item[$D$:]Generate $b\gets\bit$, $x\gets\Domprf$, and $y_0\gets\Ranprf$. Compute $y_1\gets\Eval(\prfk,x)$. Output $(b,x,y_b)$.
%\end{description}
%We also let $\cP=(P_{b,x,y},Q_{b,x,y})_{b,x,y}$ be a collection of binary outcome projective measurements, where
%\begin{align}
%P_{b,x,y}=U_{x,y}^\dagger\ket{b}\bra{b}U_{x,y}\textrm{~~~~and~~~~}Q_{b,x,y}=I-P_{b,x,y}.
%\end{align}
%Moreover, we let $\cM_D=(P_D,Q_D)$, where
%\begin{align}
%P_D=\sum_{r\in\calR}\frac{1}{\abs{\calR}}P_{D(r)}\textrm{~~~~and~~~~}Q_D=I-P_D.
%\end{align}
%We consider the following events, where $\Oracle{wprf}$ is implemented by using $\prfk$.

%\begin{description}
%\item[$\Live$:] When applying the measurement $\projimp(M_D)$ to $\rho$, we obtain a value $p$ such that $p\geq\epsilon$.
%%~\footnote{The definition would be equivalent if we use $\cM_{\tlC}^\prime$ instead of $\cM_{C}^\prime$, up to a negligible difference in $\eps$, since by statistical correctness  we have $C \cong_{\delta} \tlC$ for some $\delta = 1 -\negl(\secp)$.}\ryo{Correspond to $\qevaluator \cong_{\epsilon} C$.}
%\item[$\GoodExt$:] When Computing $\msg^\prime \lrun \qExtract^{\Oracle{wprf}}(\ek,\qstate{C}')$, it holds that $\msg^\prime \ne \unmarked$.
%\item[$\BadExt$:] When Computing $\msg^\prime \lrun \qExtract^{\Oracle{wprf}}(\ek, \qstate{C}')$, it holds that $\msg^\prime \notin \{\msg,\unmarked\}$.
%\end{description}
%

\paragraph{The proof of $\Pr[\GoodExt]\geq\Pr[\Live]-\negl(\secp)$.}
$\qExtract$ outputs $\unmarked$ only when $\tlp_{\ell+1}<\frac{1}{2}+\epsilon-\epsilon'$, that is we have $\Pr[\GoodExt]=\Pr[\tlp_{\ell+1}\geq\frac{1}{2}+\epsilon-\epsilon']$.
Let $p$ the probability obtained by applying $\projimp(\cM_D)$ to $\rho$.
Then, we have $\Pr[\Live]=\Pr[p\geq\frac{1}{2}+\epsilon]$.
Since $D$ and $D_{\ell+1}$ are computationally indistinguishable from the MDD security of $\ELWMPRF$, from \cref{thm:api_property} and \cref{cor:cind_sample_api}, we have
\begin{align}
\Pr[\Live]=\Pr[p\geq\frac{1}{2}+\epsilon]\leq\Pr[\tlp_{\ell+1}\geq\frac{1}{2}+\epsilon-4\epsilon']+\negl(\secp)=\Pr[\GoodExt]+\negl(\secp).
\end{align}






\paragraph{The proof of $\Pr[\BadExt]\leq\negl(\secp)$.}
We define the event $\BadExt_i$ as follows for every $i\in[\ell]$.
\begin{description}
\item[$\BadExt_i$:]When Running $\qExtract^{\Oracle{wprf}}(\ek,\qstate{C}')$, the following conditions hold.
\begin{itemize}
\item $\tlp_{\ell+1}\geq\frac{1}{2}+\epsilon-4\epsilon'$ holds.
\item $\msg'_j=\msg_j$ holds for every $j\in[i-1]$.
\item $\qExtract$ exits the $i$-th loop or $\msg'_i\neq\msg_i$ holds.
\end{itemize}
\end{description}
Then, we have $\Pr[\BadExt]\leq\sum_{i\in[\ell]}\Pr[\BadExt_i]$.
Below, we estimate $\Pr[\BadExt_i]$.

We first consider the case of $\msg_{i-1}=0$ and $\msg_i=0$.
Assume $\msg'_{i-1}=\msg_{i-1}=0$ holds.
Then, we have $\tlp_{i-1}>\frac{1}{2}+\epsilon-4i\epsilon'$.
Let $\tlp'_{i-1} \gets \API_{\cP,D_{i-1}}^{\epsilon' ,\delta'}(\rho_{i-1})$.
From, the almost-projective property of $\API$, we have
\begin{align}
\Pr[\tlp'_{i-1}>\frac{1}{2}+\epsilon-4i\epsilon'-\epsilon']\geq1-\delta'.
\end{align}
When $\msg_{i-1}=0$ and $\msg_i=0$, $D_{i-1}$ and $D_{i}$ are computationally indistinguishable from the MDD security of $\ELWMPRF$.
Thus, from \cref{cor:cind_sample_api}, we have
\begin{align}
1-\delta'\leq
\Pr[\tlp'_{i-1}>\frac{1}{2}+\epsilon-(4i+1)\epsilon']
\leq\Pr[\tlp_{i}>\frac{1}{2}+\epsilon-4(i+1)\epsilon']+\negl(\secp).
\end{align}
This means that $\Pr[\BadExt_i]=\negl(\secp)$ in this case.

Next, we consider the case of $\msg_{i-1}=0$ and $\msg_i=1$.
Assume $\msg'_{i-1}=\msg_{i-1}=0$ holds.
Then, we have $\tlp_{i-1}>\frac{1}{2}+\epsilon-4i\epsilon'$.
Let $\tlp'_{i-1} \gets \API_{\cP,\Drev_{i-1}}^{\epsilon' ,\delta'}(\rho_{i-1})$.
From, the reverse-almost-projective property of $\API$, we have
\begin{align}
\Pr[\tlp'_{i-1}<\frac{1}{2}-\epsilon+4i\epsilon'+\epsilon']\geq1-\delta'.
\end{align}
When $\msg_{i-1}=0$ and $\msg_i=1$, $\Drev_{i-1}$ and $D_{i}$ are computationally indistinguishable from the MDD security of $\ELWMPRF$.
Thus, from \cref{cor:cind_sample_api}, we have
\begin{align}
1-\delta'\leq
\Pr[\tlp'_{i-1}<\frac{1}{2}-\epsilon+(4i+1)\epsilon']
\leq\Pr[\tlp_{i}<\frac{1}{2}-\epsilon+4(i+1)\epsilon']+\negl(\secp).
\end{align}
This means that $\Pr[\BadExt_i]=\negl(\secp)$ also in this case.

Similarly, we can prove that $\Pr[\BadExt_i]=\negl(\secp)$ holds in the case of $(\msg_{i-1},\msg_i)=(1,0)$ and $(\msg_{i-1},\msg_i)=(1,1)$.

Overall, we see that $\Pr[\BadExt]=\negl(\secp)$ holds in all cases.




\begin{definition}[$(\epsilon,\delta)$-Reverse Almost Projective]\label{def:rev_almost_projective}
Let $\cP=(P_i,Q_i)_i$ be a collection of binary outcome projective measurements.
Let $D$ be a distribution.
We also let $\cPrev=(Q_i,P_i)_i$.
$\API$ is $(\epsilon,\delta)$-reverse almost projective if the following holds. For any quantum state $\ket{\psi}$, we apply $ \API_{\cP,D}^{\epsilon' ,\delta'}$ and $\API_{\cPrev,D}^{\epsilon' ,\delta'}$ in a row to $\ket{\psi}$ and obtain measurement outcomes $x$ and $y$, respectively. Then, $\Pr[\abs{(1-x)-y}\le \epsilon]\ge 1-\delta$.
\end{definition}
\fuyuki{We need to show that Zhandry's $\API$ satisfies this property.}


















































==> section/st_recover.tex <==
% !TEX root = ../main.tex

\newcommand{\sfEq}{\mathsf{Eq}}
\newcommand{\sfall}{\mathsf{all}}
\newcommand{\sfsub}{\mathsf{sub}}
\newcommand{\sftriv}{\mathsf{triv}}

\section{State Recovery for Expectable Outputs}\label{sec:st_recovery}
\ryo{Currently, this section is just my memo and unreadable.}
measure whether $f(x)$ is equal to $y$: Measurement $\cM_y$ to $U_x \rho U_x^\dagger$ (write the result $f(x)=y$ or not in a resulting register and measure the resulting register).

Let $V_y$ be a projection that checks if in superposition\ryo{??}, the first register is equal to $y$.
We have $P_{x,y} = V_y U_{x}$ and $Q_{x,y} = \mat{I} - P_{x,y}$.

trivial distribution?
Projective measurement $\cP= \setbk{\cP_x = (P_x,Q_x)}_{x\in \Xs}$ where $\Xs$ is the domain of function $f:\cX \ra \cY$.
Let $D$ be a distribution with random coin set $\cR$ ($\cR$ corresponds to $\cX$ in our setting).

Measurement $\cP_{x,y}=(P_{x,y},Q_{x,y})$ simply means evaluating $f$ on input $x$ and check if the resulting output is equal to $y$.

\begin{description}
\item[Distribution $D_{f,\sfall}$:]$ $
\begin{itemize}
\item Choose $x \chosen \cX$.
\item Output $(x,f(x))$.
\end{itemize}
\item[Distribution $D_{f,\sfsub,S}$:]$ $
\begin{itemize}
\item Choose $x \chosen S \subset \cX$ where $\abs{S}=\poly(\secp)$.
\item Output $(x,f(x))$.
\end{itemize}
\item[Distribution $D_{\sftriv,S}$:]$ $
\begin{itemize}
\item Choose $x \chosen S\subset \cX$ and $y \chosen \cY$ where $\abs{S}=\poly(\secp)$.
 \item Output $(x,y)$.
\end{itemize}
\end{description}

Define that the measurement outcome is $0$ means the output $f(x)$ is not equal to $y$.
If the measurement outcome is $0$ with probability $\Tr[Q_{x,y}\rho]= 1-\negl(\secp)$, we can recover a state $\rho^\prime$ such that $\trdist{\rho-\rho^\prime}\le \negl(\secp)$ by~\cref{lem:alsmot_as_good_as_new}.


